Measurement of azimuthal asymmetries in inclusive charged dipion production in $e^+e^-$ annihilations at $\sqrt{s}$ = 3.65 GeV

We present a measurement of the azimuthal asymmetries of two charged pions in the inclusive process $e^+e^-\rightarrow \pi\pi X$ based on a data set of 62 $\rm{pb}^{-1}$ at the center-of-mass energy $\sqrt{s}=3.65$ GeV collected with the BESIII detector. These asymmetries can be attributed to the Collins fragmentation function. We observe a nonzero asymmetry, which increases with increasing pion momentum. As our energy scale is close to that of the existing semi-inclusive deep inelastic scattering experimental data, the measured asymmetries are important inputs for the global analysis of extracting the quark transversity distribution inside the nucleon and are valuable to explore the energy evolution of the spin-dependent fragmentation function.

==> authors_jul2015.tex <==
\author{
  \begin{small}
    \begin{center}
      M.~Ablikim$^{1}$, M.~N.~Achasov$^{9,f}$, X.~C.~Ai$^{1}$,
      O.~Albayrak$^{5}$, M.~Albrecht$^{4}$, D.~J.~Ambrose$^{44}$,
      A.~Amoroso$^{49A,49C}$, F.~F.~An$^{1}$, Q.~An$^{46,a}$,
      J.~Z.~Bai$^{1}$, R.~Baldini Ferroli$^{20A}$, Y.~Ban$^{31}$,
      D.~W.~Bennett$^{19}$, J.~V.~Bennett$^{5}$, M.~Bertani$^{20A}$,
      D.~Bettoni$^{21A}$, J.~M.~Bian$^{43}$, F.~Bianchi$^{49A,49C}$,
      E.~Boger$^{23,d}$, I.~Boyko$^{23}$, R.~A.~Briere$^{5}$,
      H.~Cai$^{51}$, X.~Cai$^{1,a}$, O. ~Cakir$^{40A,b}$,
      A.~Calcaterra$^{20A}$, G.~F.~Cao$^{1}$, S.~A.~Cetin$^{40B}$,
      J.~F.~Chang$^{1,a}$, G.~Chelkov$^{23,d,e}$, G.~Chen$^{1}$,
      H.~S.~Chen$^{1}$, H.~Y.~Chen$^{2}$, J.~C.~Chen$^{1}$,
      M.~L.~Chen$^{1,a}$, S.~J.~Chen$^{29}$, X.~Chen$^{1,a}$,
      X.~R.~Chen$^{26}$, Y.~B.~Chen$^{1,a}$, H.~P.~Cheng$^{17}$,
      X.~K.~Chu$^{31}$, G.~Cibinetto$^{21A}$, H.~L.~Dai$^{1,a}$,
      J.~P.~Dai$^{34}$, A.~Dbeyssi$^{14}$, D.~Dedovich$^{23}$,
      Z.~Y.~Deng$^{1}$, A.~Denig$^{22}$, I.~Denysenko$^{23}$,
      M.~Destefanis$^{49A,49C}$, F.~De~Mori$^{49A,49C}$,
      Y.~Ding$^{27}$, C.~Dong$^{30}$, J.~Dong$^{1,a}$,
      L.~Y.~Dong$^{1}$, M.~Y.~Dong$^{1,a}$, S.~X.~Du$^{53}$,
      P.~F.~Duan$^{1}$, E.~E.~Eren$^{40B}$, J.~Z.~Fan$^{39}$,
      J.~Fang$^{1,a}$, S.~S.~Fang$^{1}$, X.~Fang$^{46,a}$,
      Y.~Fang$^{1}$, L.~Fava$^{49B,49C}$, F.~Feldbauer$^{22}$,
      G.~Felici$^{20A}$, C.~Q.~Feng$^{46,a}$, E.~Fioravanti$^{21A}$,
      M. ~Fritsch$^{14,22}$, C.~D.~Fu$^{1}$, Q.~Gao$^{1}$,
      X.~Y.~Gao$^{2}$, Y.~Gao$^{39}$, Z.~Gao$^{46,a}$,
      I.~Garzia$^{21A}$, K.~Goetzen$^{10}$, W.~X.~Gong$^{1,a}$,
      W.~Gradl$^{22}$, M.~Greco$^{49A,49C}$, M.~H.~Gu$^{1,a}$,
      Y.~T.~Gu$^{12}$, Y.~H.~Guan$^{1}$, A.~Q.~Guo$^{1}$,
      L.~B.~Guo$^{28}$, Y.~Guo$^{1}$, Y.~P.~Guo$^{22}$,
      Z.~Haddadi$^{25}$, A.~Hafner$^{22}$, S.~Han$^{51}$,
      X.~Q.~Hao$^{15}$, F.~A.~Harris$^{42}$, K.~L.~He$^{1}$,
      X.~Q.~He$^{45}$, T.~Held$^{4}$, Y.~K.~Heng$^{1,a}$,
      Z.~L.~Hou$^{1}$, C.~Hu$^{28}$, H.~M.~Hu$^{1}$,
      J.~F.~Hu$^{49A,49C}$, T.~Hu$^{1,a}$, Y.~Hu$^{1}$,
      G.~M.~Huang$^{6}$, G.~S.~Huang$^{46,a}$, J.~S.~Huang$^{15}$,
      X.~T.~Huang$^{33}$, Y.~Huang$^{29}$, T.~Hussain$^{48}$,
      Q.~Ji$^{1}$, Q.~P.~Ji$^{30}$, X.~B.~Ji$^{1}$, X.~L.~Ji$^{1,a}$,
      L.~W.~Jiang$^{51}$, X.~S.~Jiang$^{1,a}$, X.~Y.~Jiang$^{30}$,
      J.~B.~Jiao$^{33}$, Z.~Jiao$^{17}$, D.~P.~Jin$^{1,a}$,
      S.~Jin$^{1}$, T.~Johansson$^{50}$, A.~Julin$^{43}$,
      N.~Kalantar-Nayestanaki$^{25}$, X.~L.~Kang$^{1}$,
      X.~S.~Kang$^{30}$, M.~Kavatsyuk$^{25}$, B.~C.~Ke$^{5}$,
      P. ~Kiese$^{22}$, R.~Kliemt$^{14}$, B.~Kloss$^{22}$,
      O.~B.~Kolcu$^{40B,i}$, B.~Kopf$^{4}$, M.~Kornicer$^{42}$,
      W.~K\"uhn$^{24}$, A.~Kupsc$^{50}$, J.~S.~Lange$^{24}$,
      M.~Lara$^{19}$, P. ~Larin$^{14}$, C.~Leng$^{49C}$, C.~Li$^{50}$,
      Cheng~Li$^{46,a}$, D.~M.~Li$^{53}$, F.~Li$^{1,a}$,
      F.~Y.~Li$^{31}$, G.~Li$^{1}$, H.~B.~Li$^{1}$, J.~C.~Li$^{1}$,
      Jin~Li$^{32}$, K.~Li$^{33}$, K.~Li$^{13}$, Lei~Li$^{3}$,
      P.~R.~Li$^{41}$, T. ~Li$^{33}$, W.~D.~Li$^{1}$, W.~G.~Li$^{1}$,
      X.~L.~Li$^{33}$, X.~M.~Li$^{12}$, X.~N.~Li$^{1,a}$,
      X.~Q.~Li$^{30}$, Z.~B.~Li$^{38}$, H.~Liang$^{46,a}$,
      Y.~F.~Liang$^{36}$, Y.~T.~Liang$^{24}$, G.~R.~Liao$^{11}$,
      D.~X.~Lin$^{14}$, B.~J.~Liu$^{1}$, C.~X.~Liu$^{1}$,
      F.~H.~Liu$^{35}$, Fang~Liu$^{1}$, Feng~Liu$^{6}$,
      H.~B.~Liu$^{12}$, H.~H.~Liu$^{16}$, H.~H.~Liu$^{1}$,
      H.~M.~Liu$^{1}$, J.~Liu$^{1}$, J.~B.~Liu$^{46,a}$,
      J.~P.~Liu$^{51}$, J.~Y.~Liu$^{1}$, K.~Liu$^{39}$,
      K.~Y.~Liu$^{27}$, L.~D.~Liu$^{31}$, P.~L.~Liu$^{1,a}$,
      Q.~Liu$^{41}$, S.~B.~Liu$^{46,a}$, X.~Liu$^{26}$,
      Y.~B.~Liu$^{30}$, Z.~A.~Liu$^{1,a}$, Zhiqing~Liu$^{22}$,
      H.~Loehner$^{25}$, X.~C.~Lou$^{1,a,h}$, H.~J.~Lu$^{17}$,
      J.~G.~Lu$^{1,a}$, Y.~Lu$^{1}$, Y.~P.~Lu$^{1,a}$,
      C.~L.~Luo$^{28}$, M.~X.~Luo$^{52}$, T.~Luo$^{42}$,
      X.~L.~Luo$^{1,a}$, X.~R.~Lyu$^{41}$, F.~C.~Ma$^{27}$,
      H.~L.~Ma$^{1}$, L.~L. ~Ma$^{33}$, Q.~M.~Ma$^{1}$, T.~Ma$^{1}$,
      X.~N.~Ma$^{30}$, X.~Y.~Ma$^{1,a}$, F.~E.~Maas$^{14}$,
      M.~Maggiora$^{49A,49C}$, Y.~J.~Mao$^{31}$, Z.~P.~Mao$^{1}$,
      S.~Marcello$^{49A,49C}$, J.~G.~Messchendorp$^{25}$,
      J.~Min$^{1,a}$, R.~E.~Mitchell$^{19}$, X.~H.~Mo$^{1,a}$,
      Y.~J.~Mo$^{6}$, C.~Morales Morales$^{14}$, K.~Moriya$^{19}$,
      N.~Yu.~Muchnoi$^{9,f}$, H.~Muramatsu$^{43}$, Y.~Nefedov$^{23}$,
      F.~Nerling$^{14}$, I.~B.~Nikolaev$^{9,f}$, Z.~Ning$^{1,a}$,
      S.~Nisar$^{8}$, S.~L.~Niu$^{1,a}$, X.~Y.~Niu$^{1}$,
      S.~L.~Olsen$^{32}$, Q.~Ouyang$^{1,a}$, S.~Pacetti$^{20B}$,
      P.~Patteri$^{20A}$, M.~Pelizaeus$^{4}$, H.~P.~Peng$^{46,a}$,
      K.~Peters$^{10}$, J.~Pettersson$^{50}$, J.~L.~Ping$^{28}$,
      R.~G.~Ping$^{1}$, R.~Poling$^{43}$, V.~Prasad$^{1}$,
      M.~Qi$^{29}$, S.~Qian$^{1,a}$, C.~F.~Qiao$^{41}$,
      L.~Q.~Qin$^{33}$, N.~Qin$^{51}$, X.~S.~Qin$^{1}$,
      Z.~H.~Qin$^{1,a}$, J.~F.~Qiu$^{1}$, K.~H.~Rashid$^{48}$,
      C.~F.~Redmer$^{22}$, M.~Ripka$^{22}$, G.~Rong$^{1}$,
      Ch.~Rosner$^{14}$, X.~D.~Ruan$^{12}$, V.~Santoro$^{21A}$,
      A.~Sarantsev$^{23,g}$, M.~Savri\'e$^{21B}$,
      K.~Schoenning$^{50}$, S.~Schumann$^{22}$, W.~Shan$^{31}$,
      M.~Shao$^{46,a}$, C.~P.~Shen$^{2}$, P.~X.~Shen$^{30}$,
      X.~Y.~Shen$^{1}$, H.~Y.~Sheng$^{1}$, W.~M.~Song$^{1}$,
      X.~Y.~Song$^{1}$, S.~Sosio$^{49A,49C}$, S.~Spataro$^{49A,49C}$,
      G.~X.~Sun$^{1}$, J.~F.~Sun$^{15}$, S.~S.~Sun$^{1}$,
      Y.~J.~Sun$^{46,a}$, Y.~Z.~Sun$^{1}$, Z.~J.~Sun$^{1,a}$,
      Z.~T.~Sun$^{19}$, C.~J.~Tang$^{36}$, X.~Tang$^{1}$,
      I.~Tapan$^{40C}$, E.~H.~Thorndike$^{44}$, M.~Tiemens$^{25}$,
      M.~Ullrich$^{24}$, I.~Uman$^{40B}$, G.~S.~Varner$^{42}$,
      B.~Wang$^{30}$, D.~Wang$^{31}$, D.~Y.~Wang$^{31}$,
      K.~Wang$^{1,a}$, L.~L.~Wang$^{1}$, L.~S.~Wang$^{1}$,
      M.~Wang$^{33}$, P.~Wang$^{1}$, P.~L.~Wang$^{1}$,
      S.~G.~Wang$^{31}$, W.~Wang$^{1,a}$, X.~F. ~Wang$^{39}$,
      Y.~D.~Wang$^{14}$, Y.~F.~Wang$^{1,a}$, Y.~Q.~Wang$^{22}$,
      Z.~Wang$^{1,a}$, Z.~G.~Wang$^{1,a}$, Z.~H.~Wang$^{46,a}$,
      Z.~Y.~Wang$^{1}$, T.~Weber$^{22}$, D.~H.~Wei$^{11}$,
      J.~B.~Wei$^{31}$, P.~Weidenkaff$^{22}$, S.~P.~Wen$^{1}$,
      U.~Wiedner$^{4}$, M.~Wolke$^{50}$, L.~H.~Wu$^{1}$,
      Z.~Wu$^{1,a}$, L.~G.~Xia$^{39}$, Y.~Xia$^{18}$, D.~Xiao$^{1}$,
      H.~Xiao$^{47}$, Z.~J.~Xiao$^{28}$, Y.~G.~Xie$^{1,a}$,
      Q.~L.~Xiu$^{1,a}$, G.~F.~Xu$^{1}$, L.~Xu$^{1}$, Q.~J.~Xu$^{13}$,
      X.~P.~Xu$^{37}$, L.~Yan$^{46,a}$, W.~B.~Yan$^{46,a}$,
      W.~C.~Yan$^{46,a}$, Y.~H.~Yan$^{18}$, H.~J.~Yang$^{34}$,
      H.~X.~Yang$^{1}$, L.~Yang$^{51}$, Y.~Yang$^{6}$,
      Y.~X.~Yang$^{11}$, M.~Ye$^{1,a}$, M.~H.~Ye$^{7}$,
      J.~H.~Yin$^{1}$, B.~X.~Yu$^{1,a}$, C.~X.~Yu$^{30}$,
      J.~S.~Yu$^{26}$, C.~Z.~Yuan$^{1}$, W.~L.~Yuan$^{29}$,
      Y.~Yuan$^{1}$, A.~Yuncu$^{40B,c}$, A.~A.~Zafar$^{48}$,
      A.~Zallo$^{20A}$, Y.~Zeng$^{18}$, B.~X.~Zhang$^{1}$,
      B.~Y.~Zhang$^{1,a}$, C.~Zhang$^{29}$, C.~C.~Zhang$^{1}$,
      D.~H.~Zhang$^{1}$, H.~H.~Zhang$^{38}$, H.~Y.~Zhang$^{1,a}$,
      J.~J.~Zhang$^{1}$, J.~L.~Zhang$^{1}$, J.~Q.~Zhang$^{1}$,
      J.~W.~Zhang$^{1,a}$, J.~Y.~Zhang$^{1}$, J.~Z.~Zhang$^{1}$,
      K.~Zhang$^{1}$, L.~Zhang$^{1}$, X.~Y.~Zhang$^{33}$,
      Y.~Zhang$^{1}$, Y. ~N.~Zhang$^{41}$, Y.~H.~Zhang$^{1,a}$,
      Y.~T.~Zhang$^{46,a}$, Yu~Zhang$^{41}$, Z.~H.~Zhang$^{6}$,
      Z.~P.~Zhang$^{46}$, Z.~Y.~Zhang$^{51}$, G.~Zhao$^{1}$,
      J.~W.~Zhao$^{1,a}$, J.~Y.~Zhao$^{1}$, J.~Z.~Zhao$^{1,a}$,
      Lei~Zhao$^{46,a}$, Ling~Zhao$^{1}$, M.~G.~Zhao$^{30}$,
      Q.~Zhao$^{1}$, Q.~W.~Zhao$^{1}$, S.~J.~Zhao$^{53}$,
      T.~C.~Zhao$^{1}$, Y.~B.~Zhao$^{1,a}$, Z.~G.~Zhao$^{46,a}$,
      A.~Zhemchugov$^{23,d}$, B.~Zheng$^{47}$, J.~P.~Zheng$^{1,a}$,
      W.~J.~Zheng$^{33}$, Y.~H.~Zheng$^{41}$, B.~Zhong$^{28}$,
      L.~Zhou$^{1,a}$, X.~Zhou$^{51}$, X.~K.~Zhou$^{46,a}$,
      X.~R.~Zhou$^{46,a}$, X.~Y.~Zhou$^{1}$, K.~Zhu$^{1}$,
      K.~J.~Zhu$^{1,a}$, S.~Zhu$^{1}$, S.~H.~Zhu$^{45}$,
      X.~L.~Zhu$^{39}$, Y.~C.~Zhu$^{46,a}$, Y.~S.~Zhu$^{1}$,
      Z.~A.~Zhu$^{1}$, J.~Zhuang$^{1,a}$, L.~Zotti$^{49A,49C}$,
      B.~S.~Zou$^{1}$, J.~H.~Zou$^{1}$ 
      \\
      \vspace{0.2cm}
      (BESIII Collaboration)\\
      \vspace{0.2cm} {\it
        $^{1}$ Institute of High Energy Physics, Beijing 100049, People's Republic of China\\
        $^{2}$ Beihang University, Beijing 100191, People's Republic of China\\
        $^{3}$ Beijing Institute of Petrochemical Technology, Beijing 102617, People's Republic of China\\
        $^{4}$ Bochum Ruhr-University, D-44780 Bochum, Germany\\
        $^{5}$ Carnegie Mellon University, Pittsburgh, Pennsylvania 15213, USA\\
        $^{6}$ Central China Normal University, Wuhan 430079, People's Republic of China\\
        $^{7}$ China Center of Advanced Science and Technology, Beijing 100190, People's Republic of China\\
        $^{8}$ COMSATS Institute of Information Technology, Lahore, Defence Road, Off Raiwind Road, 54000 Lahore, Pakistan\\
        $^{9}$ G.I. Budker Institute of Nuclear Physics SB RAS (BINP), Novosibirsk 630090, Russia\\
        $^{10}$ GSI Helmholtzcentre for Heavy Ion Research GmbH, D-64291 Darmstadt, Germany\\
        $^{11}$ Guangxi Normal University, Guilin 541004, People's Republic of China\\
        $^{12}$ GuangXi University, Nanning 530004, People's Republic of China\\
        $^{13}$ Hangzhou Normal University, Hangzhou 310036, People's Republic of China\\
        $^{14}$ Helmholtz Institute Mainz, Johann-Joachim-Becher-Weg 45, D-55099 Mainz, Germany\\
        $^{15}$ Henan Normal University, Xinxiang 453007, People's Republic of China\\
        $^{16}$ Henan University of Science and Technology, Luoyang 471003, People's Republic of China\\
        $^{17}$ Huangshan College, Huangshan 245000, People's Republic of China\\
        $^{18}$ Hunan University, Changsha 410082, People's Republic of China\\
        $^{19}$ Indiana University, Bloomington, Indiana 47405, USA\\
        $^{20}$ (A)INFN Laboratori Nazionali di Frascati, I-00044, Frascati, Italy; (B)INFN and University of Perugia, I-06100, Perugia, Italy\\
        $^{21}$ (A)INFN Sezione di Ferrara, I-44122, Ferrara, Italy; (B)University of Ferrara, I-44122, Ferrara, Italy\\
        $^{22}$ Johannes Gutenberg University of Mainz, Johann-Joachim-Becher-Weg 45, D-55099 Mainz, Germany\\
        $^{23}$ Joint Institute for Nuclear Research, 141980 Dubna, Moscow region, Russia\\
        $^{24}$ Justus Liebig University Giessen, II. Physikalisches Institut, Heinrich-Buff-Ring 16, D-35392 Giessen, Germany\\
        $^{25}$ KVI-CART, University of Groningen, NL-9747 AA Groningen, The Netherlands\\
        $^{26}$ Lanzhou University, Lanzhou 730000, People's Republic of China\\
        $^{27}$ Liaoning University, Shenyang 110036, People's Republic of China\\
        $^{28}$ Nanjing Normal University, Nanjing 210023, People's Republic of China\\
        $^{29}$ Nanjing University, Nanjing 210093, People's Republic of China\\
        $^{30}$ Nankai University, Tianjin 300071, People's Republic of China\\
        $^{31}$ Peking University, Beijing 100871, People's Republic of China\\
        $^{32}$ Seoul National University, Seoul, 151-747 Korea\\
        $^{33}$ Shandong University, Jinan 250100, People's Republic of China\\
        $^{34}$ Shanghai Jiao Tong University, Shanghai 200240, People's Republic of China\\
        $^{35}$ Shanxi University, Taiyuan 030006, People's Republic of China\\
        $^{36}$ Sichuan University, Chengdu 610064, People's Republic of China\\
        $^{37}$ Soochow University, Suzhou 215006, People's Republic of China\\
        $^{38}$ Sun Yat-Sen University, Guangzhou 510275, People's Republic of China\\
        $^{39}$ Tsinghua University, Beijing 100084, People's Republic of China\\
        $^{40}$ (A)Istanbul Aydin University, 34295 Sefakoy, Istanbul, Turkey; (B)Dogus University, 34722 Istanbul, Turkey; (C)Uludag University, 16059 Bursa, Turkey\\
        $^{41}$ University of Chinese Academy of Sciences, Beijing 100049, People's Republic of China\\
        $^{42}$ University of Hawaii, Honolulu, Hawaii 96822, USA\\
        $^{43}$ University of Minnesota, Minneapolis, Minnesota 55455, USA\\
        $^{44}$ University of Rochester, Rochester, New York 14627, USA\\
        $^{45}$ University of Science and Technology Liaoning, Anshan 114051, People's Republic of China\\
        $^{46}$ University of Science and Technology of China, Hefei 230026, People's Republic of China\\
        $^{47}$ University of South China, Hengyang 421001, People's Republic of China\\
        $^{48}$ University of the Punjab, Lahore-54590, Pakistan\\
        $^{49}$ (A)University of Turin, I-10125, Turin, Italy; (B)University of Eastern Piedmont, I-15121, Alessandria, Italy; (C)INFN, I-10125, Turin, Italy\\
        $^{50}$ Uppsala University, Box 516, SE-75120 Uppsala, Sweden\\
        $^{51}$ Wuhan University, Wuhan 430072, People's Republic of China\\
        $^{52}$ Zhejiang University, Hangzhou 310027, People's Republic of China\\
        $^{53}$ Zhengzhou University, Zhengzhou 450001, People's Republic of China\\
        \vspace{0.2cm}
        $^{a}$ Also at State Key Laboratory of Particle Detection and Electronics, Beijing 100049, Hefei 230026, People's Republic of China\\
        $^{b}$ Also at Ankara University,06100 Tandogan, Ankara, Turkey\\
        $^{c}$ Also at Bogazici University, 34342 Istanbul, Turkey\\
        $^{d}$ Also at the Moscow Institute of Physics and Technology, Moscow 141700, Russia\\
        $^{e}$ Also at the Functional Electronics Laboratory, Tomsk State University, Tomsk, 634050, Russia\\
        $^{f}$ Also at the Novosibirsk State University, Novosibirsk, 630090, Russia\\
        $^{g}$ Also at the NRC ``Kurchatov Institute'', PNPI, 188300, Gatchina, Russia\\
        $^{h}$ Also at University of Texas at Dallas, Richardson, Texas 75083, USA\\
        $^{i}$ Also at Istanbul Arel University, 34295 Istanbul, Turkey\\
      }
    \end{center}
  \vspace{0.4cm}
  \end{small}
}

%\affiliation{}


